DAG-based Scheduling with Resource Sharing for Multi-task Applications in a Polyglot GPU Runtime

GPUs are readily available in cloud computing and personal devices, but their use for data processing acceleration has been slowed down by their limited integration with common programming languages such as Python or Java. Moreover, using GPUs to their full capabilities requires expert knowledge of asynchronous programming. In this work, we present a novel GPU run time scheduler for multi-task GPU computations that transparently provides asynchronous execution, space-sharing, and transfer-computation overlap without requiring in advance any information about the program dependency structure. We leverage the GrCUDA polyglot API to integrate our scheduler with multiple high-level languages and provide a platform for fast prototyping and easy GPU acceleration. We validate our work on 6 benchmarks created to evaluate task-parallelism and show an average of 44% speedup against synchronous execution, with no execution time slowdown compared to hand-optimized host code written using the C++ CUDA Graphs API.

==> tables/benchmark.tex <==
\renewcommand\theadalign{tl}
\renewcommand\theadfont{\bfseries}
\setlength\tabcolsep{5pt}
% \renewcommand\theadgape{\Gape[10pt]}
% \renewcommand\cellgape{\Gape[10pt]}

\begin{table}
\centering
\ra{1.2}
    \caption{Benchmarks in our evaluation. Input size is the number of elements in the benchmark (e.g. array sizes)}
    \resizebox{\columnwidth}{!}{
	\begin{tabular}{@{}lll@{}}
		\toprule
		\cmidrule{2-3}
		\multirow{2}{*}{\thead{Name}} & \thead{Input size\\(from - to)} & \thead{Memory\\footprint (\%)}\\
		\midrule
		
		\textbf{Vector Squares (VEC)} & $2 \cdot 10^7 - 12 \cdot 10^7$ & $17\% - 94\%$ \\
		\textbf{Black \& Scholes (B\&S)} & $2\cdot 10^6 - 12 \cdot 10^6$ & $17\% - 94\%$ \\
		\textbf{ML Ensemble (ML)} & $2 \cdot 10^5 - 12 \cdot 10^5$ & $18\% - 99\%$ \\
		\textbf{HITS} & $4 \cdot 10^6 - 20 \cdot 10^6$ & $16\% - 75\%$ \\
		\textbf{Images (IMG)} & $1600^2 - 4800^2$ & $7\% - 47\%$ \\
		\textbf{Deep Learning  (DL)} & $3000^2 - 7000^2$ & $13\% - 63\%$ \\
	
		\bottomrule
	\end{tabular}
    }
    \label{tab:benchmark}
\end{table}

==> tables/benchmark_2.tex <==
\renewcommand\theadalign{tl}
\renewcommand\theadfont{\bfseries}
\setlength\tabcolsep{5pt}
% \renewcommand\theadgape{\Gape[10pt]}
% \renewcommand\cellgape{\Gape[10pt]}

\begin{table}
\centering
\ra{1.2}
    \caption{Percentage of device memory for different input sizes in each benchmark. \glspl{gpu} are tested with different input sizes up to the largest size that fits in \gls{gpu} memory.
    % Input sizes are different on each \gls{gpu} and are chosen to provide similar percentage memory footprint.
    }
    
    \resizebox{\columnwidth}{!}{
	\begin{tabular}{@{}llll@{}}
		\toprule
		& \multicolumn{3}{c}{Memory footprint (\%)} \\
		\cmidrule{2-4}
		\thead{Benchmark name} & \thead{GTX 960} &  \thead{GTX 1660 Super} & \thead{Tesla P100} \\
		\midrule
		
		\textbf{Vector Squares (VEC)} & $17\% - 94\%$ & $18\% - 53\%$ & $18\% - 90\%$ \\
		\textbf{Black \& Scholes (B\&S)}  & $17\% - 94\%$ & $18\% - 53\%$ & $19\% - 90\%$ \\
		\textbf{Images (IMG)} & $7\% - 47\%$ & $16\% - 57\%$ & $9\% - 75\%$ \\
		\textbf{ML Ensemble (ML)}  & $18\% - 99\%$ & $14\% - 72\%$ & $19\% - 82\%$ \\
		\textbf{HITS} & $16\% - 75\%$ & $12\% - 85\%$ & $13\% - 82\%$ \\
		\textbf{Deep Learning  (DL)} & $13\% - 63\%$ & $16\% - 94\%$ & $83\% - 53\%$ \\
		
	    \midrule
	    \textbf{GPU device memory} & 2002 MB & 5944 MB & 12198 MB \\
	    
		\bottomrule
	\end{tabular}
    }
    \label{tab:benchmark}
\end{table}
